Prompting the Unseen: Detecting Hidden Backdoors in Black-Box Models

Visual prompting (VP) is a new technique that adapts well-trained frozen models for source domain tasks to target domain tasks. This study examines VP's benefits for black-box model-level backdoor detection. The visual prompt in VP maps class subspaces between source and target domains. We identify a misalignment, termed class subspace inconsistency, between clean and poisoned datasets. Based on this, we introduce \textsc{BProm}, a black-box model-level detection method to identify backdoors in suspicious models, if any. \textsc{BProm} leverages the low classification accuracy of prompted models when backdoors are present. Extensive experiments confirm \textsc{BProm}'s effectiveness.

==> sec/checklist.tex <==

\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction clearly outline the core contributions of the paper: identifying class subspace inconsistency in backdoored models under visual prompting and proposing \textsc{BProm}, a novel black-box detection method that exploits this inconsistency. The scope of the paper is limited to model-level backdoor detection.


\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The conclusion explicitly acknowledges the limitation of \textsc{BProm} in handling all-to-all backdoors caused by controllable feature space distortions. Future work to address this limitation is recommended.

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper focuses on an empirical study of a novel backdoor detection method and does not introduce theoretical claims that require formal proofs.

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper offers comprehensive details on datasets, model architectures, attack methods, defense baselines, and hyperparameter settings employed in the experiments. Furthermore, the code will be made available upon publication, enhancing the reproducibility of the primary results.
    
\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper utilizes publicly available datasets and attack/defense implementations from the Backdoor Toolbox, with links to these resources provided. Furthermore, the code for \textsc{BProm} will be openly accessible upon publication, guaranteeing complete reproducibility of the experimental results.

\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper details the training and test details, including data splits, hyperparameter choices, optimizer type, and evaluation metrics, in Section 6 (Experimental Setup) and further elaborates on attack configurations and defense configurations in Section A (Implementation Details) of the Appendix.

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper predominantly employs AUROC and F1 score as evaluation metrics, which inherently offer a measure of statistical performance across multiple trials. Furthermore, Section 6.3 (Hyperparameter Study) investigates the influence of different model and attack parameters on detection performance.
    
\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The compute resources are reported in Section~\ref{sec:Experimental Setup}.
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research adheres to the NeurIPS Code of Ethics by concentrating on enhancing security against backdoor attacks and promoting the responsible use of deep learning models.

    

\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper explores the positive societal implications of enhancing the trustworthiness and security of deep learning models, especially in MLaaS scenarios. It emphasizes the potential adverse effects of backdoor attacks and stresses the significance of robust detection.
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper presents a detection method for backdoor attacks and avoids releasing data or models that pose a direct risk of misuse.
    
\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper appropriately acknowledges the creators and sources of all datasets, model architectures, and attack/defense implementations, providing relevant citations and URLs. It also mentions utilizing the default settings and configurations from the Backdoor Toolbox, which is publicly available under an open-source license.
    
\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper introduces a novel method (\textsc{BProm}) and plans to release the accompanying code under a suitable open-source license. Documentation will accompany the code to aid in its usage and comprehension.
    
\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This research is purely computational and does not involve crowdsourcing or human subjects.

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This research is solely computational and does not involve human subjects; hence, IRB approval is not applicable.

\end{enumerate}

==> tbls/attack_configure.tex <==

\begin{table}[h]
\caption{Configurations of baseline attacks}
\label{tab:attack_config}
\centering
\footnotesize

\begin{adjustbox}{max width=1.0\columnwidth}
\begin{tabular}{lll}
\toprule
\textbf{Attacks} & \textbf{Configuration} \\
\midrule
BadNets~\cite{Gu2017BadNetsIV} & Target class: 0 \\
& Pattern: 4x4 random noise \\
% & Poison rate: 10\% \\
\midrule

Blend~\cite{Chen2017TargetedBA}   & Target class: 0 \\
& Pattern: 4x4 random noise \\
% & Poison rate: 10\% \\
\midrule

Trojan~\cite{Liu2018TrojaningAO} & Target class: 0 \\
& Pattern: square patch \\
% & Poison rate: 10\% \\
\midrule

SIG~\cite{8802997}     & Target class: 0 \\
& Pattern: 8x8 transparency-optimized noise \\
% & Poison rate: 5\% \\
\midrule

WaNet~\cite{Nguyen2021WaNetI}   & Target class: 0 \\
& Pattern: warping transform \\
% & Poison rate: 20\% \\
\midrule

Dynamic~\cite{input-aware} & Target class: 0 \\
& Pattern: sample-specific \\
% & Poison rate: 10\% \\
\midrule

TaCT~\cite{scan} & Target class: 0 \\
& Pattern: square patch \\
% & Poison rate: 10\% \\
\midrule

Adap-Blend~\cite{revisitingbackdoor} & Target class: 0 \\
& Pattern: blended random image \\
% & Poison rate: 10\% \\
\midrule

Adap-Patch~\cite{revisitingbackdoor} & Target class: 0 \\
& Pattern: random patch \\
% & Poison rate: 10\% \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tbls/detection_metrics.tex <==
\begin{table}[ht]
\centering
\caption{Summary of detection performance metrics.}
\label{tab:detection_metrics}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Attack} & \multicolumn{2}{c}{F1} & \multicolumn{2}{c}{AUCROC} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& Backdoored & Benign & Backdoored & Benign \\
\midrule
BadNet & 0.8014 & 0.5263 & 0.8113 & 0.4509 \\
Blended & 0.7621 & 0.5263 & 0.7259 & 0.3954 \\
Dynamic & 0.9407 & 0.5263 & 0.9312 & 0.4921 \\
Sig & 0.6571 & 0.5263 & 0.7214 & 0.4492 \\
WaNet & 0.9295 & 0.5263 & 0.9345 & 0.4406 \\
\bottomrule
\end{tabular}
\end{table}

